Searchable Hidden Intermediates for End-to-End Models of Decomposable Sequence Tasks

End-to-end approaches for sequence tasks are becoming increasingly popular. Yet for complex sequence tasks, like speech translation, systems that cascade several models trained on sub-tasks have shown to be superior, suggesting that the compositionality of cascaded systems simplifies learning and enables sophisticated search capabilities. In this work, we present an end-to-end framework that exploits compositionality to learn searchable hidden representations at intermediate stages of a sequence model using decomposed sub-tasks. These hidden intermediates can be improved using beam search to enhance the overall performance and can also incorporate external models at intermediate stages of the network to re-score or adapt towards out-of-domain data. One instance of the proposed framework is a Multi-Decoder model for speech translation that extracts the searchable hidden intermediates from a speech recognition sub-task. The model demonstrates the aforementioned benefits and outperforms the previous state-of-the-art by around +6 and +3 BLEU on the two test sets of Fisher-CallHome and by around +3 and +4 BLEU on the English-German and English-French test sets of MuST-C.

==> images/error_propagation.tex <==
\begin{tikzpicture}
\begin{axis}[
    ybar,
    ymax=40,
    enlarge x limits=0.25,
    bar width=18pt,
    ylabel={ST BLEU Score ($\uparrow$)},
    xlabel={ASR \% WER ($\downarrow$)},
    symbolic x coords={$<40\%$,$\rinterval{40}{80}\%$,$\geq80\%$},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    legend cell align={left},
    xlabel near ticks,
    ylabel near ticks,
    ytick align=outside,
    ytick pos=left,
    xtick align=inside,
    xtick style={draw=none},
    ]
\addplot coordinates {($<40\%$,29.8) ($\rinterval{40}{80}\%$,18.3) ($\geq80\%$,5.0)};
\addplot coordinates {($<40\%$,31.3) ($\rinterval{40}{80}\%$,15.6) ($\geq80\%$,5.0)};
\addplot coordinates {($<40\%$,32.8) ($\rinterval{40}{80}\%$,17.7) ($\geq80\%$,5.5)};
\legend{Baseline,Multi-Decoder,Multi-Decoder w/ SA}
\end{axis}
\end{tikzpicture}
